Multi-scale Online Learning and its Applications to Online Auctions

We consider revenue maximization in online auction/pricing problems. A seller sells an identical item in each period to a new buyer, or a new set of buyers. For the online posted pricing problem, we show regret bounds that scale with the best fixed price, rather than the range of the values. We also show regret bounds that are almost scale free, and match the offline sample complexity, when comparing to a benchmark that requires a lower bound on the market share. These results are obtained by generalizing the classical learning from experts and multi-armed bandit problems to their multi-scale versions. In this version, the reward of each action is in a different range, and the regret w.r.t. a given action scales with its own range, rather than the maximum range.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
Consider the following revenue maximization problem in a repeated setting, 
called the \emph{online posted pricing} problem. 
In each period, the seller has a single item to sell, and a new prospective buyer. 
The seller offers to sell the item to the buyer at a given price; 
the buyer buys the item if and only if the price is below his private valuation for the item. 
The private valuation of the buyer itself is never revealed to the seller. 
How should a monopolistic seller iteratively set the prices if he wishes to maximize his revenue? What if he also cares about market share? 

Estimating price sensitivities and demand models in order to optimize 
revenue and market share is the bedrock of econometrics. 
The emergence of online marketplaces has enabled sellers to costlessly change prices, 
as well as collect huge amounts of data. 
This has renewed the interest in understanding best practices for data driven pricing. 
The extreme case of this when the price is updated for each buyer is the {online pricing} problem described above;
one can always use this for less frequent price updates. 
Moreover this problem is intimately related to classical experimentation and estimation procedures. 

This problem has been studied from an\emph{ online learning} perspective, as a variant of 
the {\em multi-armed bandit} problem. 
The revenue of a pricing algorithm is compared to 
the revenue of the best fixed posted price, in hindsight. 
The difference between the two, called the \emph{regret}, is then bounded by above. 
No assumption is made on the distribution of values; 
the regret bounds are required to hold for the \emph{worst case} sequence of values. 
\citet{blum2004online} assume that the buyer valuations are  in $[1,h]$, and show the following multiplicative plus additive bound on the regret: 
for any $\epsilon \in (0,1)$, the regret is at most 
$\epsilon $ times the revenue of the optimal price, 
$+ ~O(\epsilon^{-2}h \log h \log\log h)$. 
\citet{blum2005near} show that the additive factor can be made to be $O(\epsilon^{-3}h  \log\log h)$, 
trading off a $\log h$ factor for an extra $\epsilon^{-1}$ factor.
%\nikhil{Lower bounds for the pricing problem?}

An undesirable aspect of these bounds is that they scale \emph{linearly with} $h$;
this is particularly problematic when $h$ is an estimate and we might set it to be a generous upper bound on the range of prices we wish to consider. 
A typical use case is when the same algorithm is used for many different products,
with widely varying price ranges. 
We may not be able to manually tune the range for each product separately. 

This dependence on $h$ seems unavoidable, as is reflected by the lower bounds for the problem. (Lower bounds are discussed later in the introduction.) 
Yet, somewhat surprisingly, \textbf{our first contribution in this paper is to show that we can get regret proportional to the best fixed price instead of the highest value for the oline posted pricing problem}. (I.e., we can replace $h$ by the best fixed price,\footnote{Standard bounds allow regret to depend on the loss of the best action instead of the worst case loss. However, even such bounds still depend linearly on the range of the losses, and thus they would not allow to replace $h$ by the best fixed price.} which is used in the definition of the benchmark.)
In particular, we show that the additive bound can be made to be $O(\epsilon^{-2} p^* \log h)$, where $p^*$ is the best fixed price in hindsight. 
This allows us to use a very generous estimate for $h$ and let the algorithm adapt to the actual range of prices; 
we only lose a $\log h$ factor.
The algorithm balances exploration probabilities of different prices carefully and automatically zooms in on the relevant price range. 
This does not violate known lower bounds, since in those instances $p^*$ is close to $h$. 

\citet{bar2002incentive}, \citet{blum2004online}, and \citet{blum2005near} also consider the ``full information''  version of the problem, or what we call the \emph{online (single buyer) auction} problem, where 
the valuations of the buyers are revealed to the algorithm after the buyer has made a decision. 
Such information may be available in a context where the buyers have to bid for the items, and are awarded the item if their bid is above a hidden price. 
In this case, the additive term can be improved to $O(\epsilon^{-1} h \log (\epsilon^{-1}))$, which is tight. 
Once again, \emph{we show that  $h$  can be replaced with} $p^*$; 
in particular, we show that the additive term can be made to be $O(\epsilon^{-1}p^* \log(h\epsilon^{-1}))$.

\subsection{Purely multiplicative bounds and sample complexity}
 The regret bounds mentioned above can be turned into a purely multiplicative factor in the following way: for any $\epsilon > 0$, the algorithm is guaranteed to get a $1-O(\epsilon)$ fraction of the best fixed price revenue, 
 provided the number of periods $T \geq E/\epsilon,$
 where $E$ is the additive term in the regret bounds above. 
 This follows from the observation that a revenue of $T$ is a lower bound on the best fixed price revenue. 
Define the number of periods required to get a $1-\epsilon$ multiplicative approximation (as  a function of $\epsilon$) to be  the \emph{convergence rate} of the algorithm. 
 
A $1-\epsilon$ multiplicative factor is also the target in the recent line of work, on the \emph{sample complexity} of auctions, started by \citet{Dhangwatnotai2014revenue,ColeR14}. 
(We give a more comprehensive discussion of this line of work in Section~\ref{sec:related-work}.)
Here,\emph{ i.i.d.} samples of the valuations are given from a \emph{fixed but unknown distribution}, and the goal is to find a price such that its revenue w.r.t.\ the hidden distribution is a 
$1-\epsilon$ fraction of the optimum revenue for this distribution. 
The sample complexity is the minimum number of samples needed to guarantee this (as a function of $\epsilon$).

The sample complexity and the convergence rate (for the full information setting) are closely related to each other. 
The sample complexity is always smaller than the convergence rate: the problem is easier because of the following. 
\begin{enumerate}
	\item The valuations are i.i.d. in case of sample complexity whereas they can be arbitrary (worst case) in case of convergence rate.  
	\item Sample complexity corresponds to an offline problem: you get all the samples at once. Convergence rate corresponds to an online problem: you need to decide what to do on a given valuation without knowing what valuations arrive in the future.
\end{enumerate}
This is formalized in terms of an \emph{online to offline reduction} [folklore]
which shows  that a convergence rate upper bound can be automatically translated to a sample complexity upper bound.
%\footnote{ 
 %As an immediate corollary, we observe that we get an improved sample complexity bound of  $O(\epsilon^{-2} h \log (\epsilon^{-1}))$ when the values are in $[1,h]$; 
 %the previous best known sample complexity bound for this case was $O(\epsilon^{-2} h \log (h \epsilon^{-1}))$ \cite{balcan2008reducing,huang2015making}. }
This lets us convert sample complexity lower bounds into lower bounds on the convergence rate, and in turn into lower bounds on the additive error $E$  in an additive plus multiplicative regret bound. 
For example, the additive error for the  online auction problem (and hence also for the posted pricing problem\footnote{
	We conjecture that the lower bound for the posted pricing problem should be worse by a factor of $\epsilon^{-1}$, since one needs to explore about $\epsilon^{-1}$ different prices. 
	%This is an interesting open problem.
}) cannot be $o(h\epsilon^{-1})$~\citep{huang2015making}. 
Moreover, it is insightful to compare convergence rates we show with {\em the best known sample complexity upper bound;  proving better convergence rates would mean improving these bounds as well}. 

A natural target convergence rate for a problem is therefore the corresponding sample complexity, but achieving this is not always trivial. 
% In many cases, the best known convergence rates are exactly the same as the best known sample complexity.
%\nikhil{Is sample complexity always smaller?}
%For instance, the convergence rate of $\epsilon^{-2}h \log (\epsilon^{-1})$, obtained as detailed earlier, 
%is also the best known sample complexity for the single item single buyer case. 
An interesting version of the sample complexity bound for auctions did not have an analogous convergence rate bound. 
 This version takes into account \emph{both revenue and market share}, and surprisingly, gets sample complexity bounds that are \emph{scale free}; 
there is no dependence on $h$, which means it works for unbounded valuations!
For any $\delta \in (0,1)$, the best fixed price benchmark is relaxed to ignore those prices whose market share (which is equivalent to the probability of sale) is below a 
$\delta $ fraction; as $\delta$ increases the benchmark is lower.
This is a meaningful benchmark since in many cases revenue is not the only goal, even if you are a monopolist.
A more reasonable goal is to maximize revenue subject to 
the constraint that the market share is above a certain threshold.
What is more, this gives a sample complexity of $O(\epsilon^{-2}\delta^{-1}\log (\delta^{-1} \epsilon^{-1}))$~\citep{huang2015making}. 
In fact $\delta$ can be set to $h^{-1}$ without loss of generality, when the values are in $[1,h]$,\footnote{\label{fn1}
	When the values are in $[1,h]$, we can guarantee a revenue of $T$ by posting  a price of 1, and to beat this, any other price (and in particular a price of $h$) would have to sell at least $T/h$ times.
} 
and the above bound then matches the sample complexity w.r.t. the best fixed price revenue.
In addition, this bound gives a precise interpolation:  
as the target market share $\delta$ increase, the number of samples needed decreases almost linearly. 

\textbf{ The second contribution of this paper is to show a convergence rate that 
almost matches the above sample complexity, for the full information setting}. 
We have a mild dependence on $h$; the rate is proportional to $\log\log h$. 
Further, we also show a near optimal convergence rate for the online posted pricing problem.\footnote{
Unfortunately, we cannot yet guarantee that our online algorithm itself gets a market share of $\delta$, although we strongly believe that it does. Showing such bounds on the market share of the algorithm is an important avenue for future research.}  


\paragraph{Multiple buyers:}
All of our results in the full information (online auction) setting extend to the multiple buyer model.
In this  model, in each time period, a new set of $n$ buyers competes for a single item. 
The seller runs a truthful auction that determines the winning buyer and his payment. 
The benchmark here is the set of all ``Myerson-type'' mechanisms. 
These are mechanisms that are optimal when each period has $n$ buyers of potentially different types, and the value of each buyer is drawn independently from a type dependent distribution.
In fact, our convergence rates also imply new sample complexity bounds for these problems 
(except that they are not computationally efficient). 
%by  \citet{devanur2016sample}, up to a $\log \log h$ factor.  
 
 The various bounds and comparisons to previous work are summarized in Tables~\ref{tab:opt} \& \ref{tab:opt-delta}. 
 
 \begin{table}[ht]
 
 	\renewcommand\arraystretch{1.5}
	\renewcommand{\thefootnote}{\fnsymbol{footnote}}
	\centering
 	\small
 	\resizebox{\textwidth}{!} {%

 	\begin{tabular}{|c|c|c|c|c|}
 		\hline
 		& \multirow{2}{*}{\shortstack{Lower bound }} & \multicolumn{3}{|c|}{Upper bound} \\
 		\cline{3-5}
 		& & \shortstack{Best known \\(Sample complexity) }& \shortstack{Best known \\ (Convergence rate)} & \shortstack{This paper \\(Thm.~\ref{thm:multadditivebounds}) }\\
 		\hline
 		Online single buyer auction & 
 		$\Omega\big(\frac{h}{\epsilon^2}\big)$~~\footnotemark[1] & 
 		$\tilde{O}\big(\frac{h}{\epsilon^2}\big)$ ~~\footnotemark[2] &
 		$\tilde{O}\big(\frac{h}{\epsilon^2}\big)$~~\footnotemark[2] & $\tilde{O}\big(\frac{\pbest}{\epsilon^2}\big)$ \\
 		\hline
 		Online posted pricing & $\Omega\big( \max\{ \frac{h}{\epsilon^2}, \frac{1}{\epsilon^3} \} \big)$~~\footnotemark[1]\footnotemark[4] & - & 
 		$\tilde{O}\big(\frac{h}{\epsilon^3}\big)$~~\footnotemark[2] & $\tilde{O}\big(\frac{\pbest}{\epsilon^3}\big)$ \\
 		\hline
 		Online multi buyer auction & $\Omega(\frac h {\epsilon^2})$~~\footnotemark[1] & 
 		$O(\frac{nh}{\epsilon^3})$ ~~\footnotemark[3] & - & $\tilde{O}\big(\frac{n h}{\epsilon^3}\big)$\\
 		\hline
 	\end{tabular}
 	}
 	\smallskip
 	
 	\noindent
 	\begin{minipage}{\textwidth}
 		{
 			\footnotesize
 			\footnotemark[1]~~{\citet{huang2015making}};~~
 			\footnotemark[2]~~{\citet{blum2004online}};~~
% 			\footnotemark[3]~~{\cite{blum2005near}}; \quad
\footnotemark[3]~~{\citet{devanur2016sample,gonczarowski2016efficient}};~~
\footnotemark[4]~~{\citet{kleinberg2003value}}.
 		}
 	\end{minipage}
 	
 	\smallskip
 	
 	\caption{Number of rounds/samples needed to get a $1-\epsilon$ approximation to the best offline price/mechanism. Sample complexity is for the offline case with i.i.d. samples from an unknown distribution. 
 		Convergence rate is for the online case with a worst case sequence. 
 		Sample complexity is always no larger than the convergence rate. 
 		Lower bounds hold for sample complexity too, except for the online posted pricing problem for which there is no sample complexity version. The additive plus multiplicative regret bounds are converted to convergence rates by dividing the additive error by $\epsilon$. 
 		In the last row, $n$ is the number of buyers. 
 	In the last column, 	$\pbest$ denotes the optimal price. }
 	
 	\vspace{2mm}
 	\label{tab:opt}
	
 	\begin{tabular}{|c|c|c|c|}
 		\hline
 		& \multirow{2}{*}{\shortstack{Lower bound \\(Sample complexity)}} & \multicolumn{2}{|c|}{Upper bound} \\
 		\cline{3-4}
 		& & \shortstack{Best known \\(Sample complexity) }& \shortstack{This paper \\(Thm.~\ref{thm:convergencerates}) }\\
 		\hline
 		Online single buyer auction & 
 		$\Omega\big(\frac{1}{\epsilon^2 \delta}\big)$~~\footnotemark[1] & 
 		$\tilde{O}\big(\frac{1}{\epsilon^2 \delta}\big)$~~\footnotemark[1] & $\tilde{O}\big(\frac{1}{\epsilon^2 \delta}\big)$ \\
 		\hline
 		Online posted pricing & $\Omega\big(\max\{ \frac{1}{\epsilon^2 \delta}, \frac{1}{\epsilon^3} \}\big)$~~\footnotemark[1]\footnotemark[2] & - & $\tilde{O}\big(\frac{1}{\epsilon^4 \delta}\big)$ \\
 		\hline
 		Online multi buyer auction & 	$\Omega\big(\frac{1}{\epsilon^2 \delta}\big)$~~\footnotemark[1] & - & $\tilde{O}\big(\frac{n}{\epsilon^3 \delta}\big)$\\
 		\hline
 	\end{tabular}
 	
 	\smallskip
 	
 	\noindent\par
 	\begin{minipage}{0.65\textwidth}
 		{
 			\footnotesize
 			\footnotemark[1]~~{\citet{huang2015making}};\quad
			\footnotemark[2]~~{\citet{kleinberg2003value}}.
 		}
 	\end{minipage}
 	
 	\smallskip
 	
 	\caption{Sample complexity \& convergence rate w.r.t.\  the opt mechanism/price with market share $\geq\delta$.}
 	\label{tab:opt-delta}
 \end{table}
 
 \iffalse 
 \noindent
%\begin{minipage}{\textwidth}
 \begin{table}[ht]
 	\centering
 	%\caption{My caption}
 	

% 		\begin{center}
 		%\begin{table}
 		\caption{Comparison of convergence rates and Sample Complexity bounds}
		\label{tab:summary}
% 		\medskip
 		\begin{tabular}{|c|c|c|c|c|}
 			\hline
 			{\bf Model}  & {\bf Sample Complexity for $v \in [1,h]$} & {\bf Convergence rate for $v \in [1,h]$ } & {\bf Sample Complexity with $\delta$ market share }& {\bf Convergence rate for $\delta$ market share} \\
 			\hline
 			  Posted Price & na & N/A &  $\Omega\left( h\epsilon^{-2}\right)$  \cite{HuangMR15} &  $ O  \left( h{\epsilon^{-3} \log h \log log h} + \log (\epsilon^{-1}) \right) $ \cite{blum2004online}\\
 			\hline
 			  Single buyer auction& ??&  Regular &  $\Omega\left( \max\{ n\epsilon^{-1}, \epsilon^{-3}\}\right)$  \cite{ColeR14,HuangMR15} &   $ \tilde{O}  \left( {n}{\epsilon^{-4}} \right)$ ({sec:no_signal})\\	\hline
 				Many buyer auctions &  ??& Regular, $q$ bounded tail & $ \Omega \left( {\epsilon^{-4}}{\log\left( \tfrac 1 {q(\epsilon)} \right) }\right) $   (Section \ref{app:signal_lb}) &  $ O  \left(  {q(\epsilon)^{-1} \epsilon^{-3}{\log (\tfrac 1 \epsilon) }}\right) $ ({sec:signal_ub_single_agent}) \\
 			\hline
 			% $n$ & Regular, $q$ bounded tail &     &  $ \tilde{O}  \left( {n^2} {q(\epsilon)^{-1} \epsilon^{-4} } \right) $ ({sec:signal_ub_multi})\\
 			\hline
 		\end{tabular}

 	%\end{center}

 \end{table}
% \end{minipage}
 \vspace{5pt}
 \fi 

\vspace{-2mm}
\subsection{Multi-scale online learning}
The main technical ingredients in our results are variants of the classical problems of learning from expert advice and multi-armed bandit. 
We introduce the multi-scale versions of these problems, 
where each action has its reward bounded in a different range. 
\textbf{Our third contribution is to give an algorithm for this problem whose regret w.r.t. a certain action scales with the range of rewards for that particular action. }
To contrast,  the regret bounds in the standard versions scale with the maximum range. 
We expect such bounds to be of independent interest. 

The multi-scale versions of these problems exhibit subtle variations that don't appear in the standard versions. 
First of all, our applications to auctions and pricing have non-negative rewards, and 
this actually makes a difference. 
For both the expert and the bandit versions, the minimax regret bounds for non-negative rewards are \emph{provably better} than those when rewards could be negative.
Further, for the bandit version, we can prove a better bound if we only 
require the bound to hold w.r.t. the \emph{best} action, rather than \emph{all} actions (for non-negative rewards). The various regret bounds and comparison to standard bounds are summarized in Tables~\ref{tab:multi-scale}.
%Whether there is really a gap between these two versions is an interesting open problem. 
\begin{table}[ht]
\renewcommand\arraystretch{1.5}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 	\small
\centering
 	\begin{tabular}{|c|c|c|c|}
 		\hline
 		& \multirow{2}{*}{\shortstack{Standard \\regret bound $O(\cdot)$}} & \multicolumn{2}{|c|}{Multi-scale bound (this paper)} \\
 		\cline{3-4}
 		& & \shortstack{Upper bound  $O(\cdot)$ }& \shortstack{Lower bound  $\Omega(\cdot)$}\\
 		\hline
 		Experts/non-negative  & 
 		$ \range_{\max}\sqrt{T\log(k)}$~~\footnotemark[1] & 
 		$ \range_{i}\sqrt{T\log(kT)} $ & $ \range_{i}\sqrt{T\log(k)} $ \\
 		\hline
 		 \multirow{2}{*}{Bandits/non-negative} &  \multirow{2}{*}{$\range_{\max}\sqrt{Tk}$~~\footnotemark[2]} & $ \range_{i} T^{\frac{2}{3}}(k\log(kT))^{\frac{1}{3}} $ &  $c_i\sqrt{TK}$\\
 		 \cline{3-4} &&$\range_{i^*}\sqrt{Tk\log(k)} $, $i^*$ is the best action & -\\
 		\hline
 		Experts/symmetric & 	$\range_{\max}\sqrt{T\log(k)}$~~\footnotemark[1] & $ \range_{i}\sqrt{T\log (k\cdot \frac{\range_{\max}}{\range_{\min}})} $ & $\range_{i}\sqrt{T\log(k)} $ \\
 		\hline
 		Bandits/symmetric & 	$\range_{\max}\sqrt{Tk}$~~\footnotemark[2] & $ \range_{i}\sqrt{Tk\cdot \frac{\range_{\max}}{\range_{\min}}\log (k T\cdot \frac{\range_{\max}}{\range_{\min}})} $ & 
 		 $ \range_{i}\sqrt{Tk\cdot \frac{\range_{\max}}{\range_{\min}}}$ \\
 		\hline
 	\end{tabular}
 		
 	\smallskip
 	
\noindent\par
 	\begin{minipage}{0.6\textwidth}
 		{
 			\center
 			\footnotesize
 			\footnotemark[1]~~{\citet{freund1995desicion}};\quad
 			\footnotemark[2]~~{\citet{audibert2009minimax}}.
 		}
 	\end{minipage}
 	
 	\smallskip
 	
 	\caption{Pure-additive regret bounds for non-negative rewards, i.e. when reward of any action $i$ at any time is in $[0,c_i]$, and symmetric range rewards, i.e. when reward of any action $i$ at any time is in $[-c_i,c_i]$ (suppose $T$ is the time horizon, $\actions$ is the action set, and $k$ is the number of actions).}
 	\label{tab:multi-scale}
 \end{table}

 We use algorithms based on online (stochastic) mirror descent (OSMD) \citep{bubeck2011introduction}, 
 with a weighted negative entropy as the Legendre function. 
This framework gives regret bounds in terms of a ``local norm'' as well as an ``initial divergence'', 
which we then bound differently for each version of the problem. 
In the technical sections we highlight how the subtle variations arise as a result 
of different techniques used to bound these two terms. 
 

\citet{foster}  also consider the multi-scale online learning problem motivated by a model selection problem.
 They consider additive bounds, for the symmetric case, for full information, but not bandit feedback. 
Their regret bounds are not comparable to ours in general; 
our bounds are better for the pricing/auction applications we consider, 
and their bounds are better for their application. 



 \subsection{Other related work}
 \label{sec:related-work} 
The online pricing problem, also called \emph{dynamic pricing}, is a much studied topic, across disciplines such as operations research and management science \citep{talluri2006theory}, economics \citep{segal2003optimal}, marketing, and of course computer science. 
The multi-armed bandit approach to pricing is particularly popular. 
  See \citet{den2015dynamic} for a recent survey on various approaches to the problem. 
  
  \citet{kleinberg2003value} consider the online pricing problem, under the assumption that the values are in $[0,1]$,  and considered purely additive factors. 
  They showed that the minimax additive  regret is $\tilde{\Theta}(T^{2/3})$, where $T$ is the number of periods. 
  This is similar in spirit to regret bounds that scale with $h$, since one has to normalize the values 
  so that they are in $[0,1]$.  
   The finer distinction about the magnitude of the best fixed price is absent in this work. 
Recently, \citet{syrgkanis2017sample} also consider the online auction problem, with an emphasis on 
a notion of ``oracle based'' computational efficiency. 
They assume the values are all in $[0,1]$ and don't consider the scaling issue that we do;
 this makes their contribution orthogonal to ours. 

Starting with \citet{Dhangwatnotai2014revenue}, there has been a spate of recent results analyzing the sample complexity of pricing and auction problems. 
\citet{ColeR14} and \citet{devanur2016sample} consider multiple buyer auctions with regular distributions (with unbounded valuations) and give sample complexity bounds that are polynomial in $n$ and $\epsilon^{-1}$, where $n$ is the number of buyers. 
\citet{MR15} consider arbitrary distributions with values bounded by $h$, and gave bounds that are polynomial in $n,h,$ and $\epsilon^{-1}$. 
\citet{roughgarden2016ironing,huang2015making} give further improvements on the single- and multi-buyer versions respectively;
Tables~\ref{tab:opt} and \ref{tab:opt-delta} give a comparison of these results with our bounds, for the problems we consider. 
The dynamic pricing problem has also been studied when there are a given number of copies of the item to sell (limited supply) \citep{agrawal2014bandits,babaioff2015dynamic,badanidiyuru2013bandits,besbes2009dynamic}. 
There are also variants where the seller interacts with the same buyer repeatedly, and the buyer can strategize to influence his utility in the future periods \citep{amin2013learning,devanur2014perfect}. 


%\citet{foster} independently consider multi-scale versions of the experts (but not the bandit) problem, but focus on purely additive factors. Their results are similar to ours in spirit, but are not exactly comparable. %\nikhil{Check this.}


\paragraph{Organization} We start in Section~\ref{sec:learning} by showing regret upper bounds for the multi-scale experts problem with non-negative rewards (Theorem \ref{thm:expert-regret-bound-rewards}). The corresponding upper bounds for the bandit version are in section \ref{sec:bandit} (Theorem~\ref{thm:bandit-regret-bound}). In Section~\ref{sec:auction} we show how the multi-scale regret bounds (Theorems \ref{thm:expert-regret-bound-rewards} and \ref{thm:bandit-regret-bound}) 
  imply the  corresponding bounds for the auction/pricing problems (Theorems \ref{thm:multadditivebounds} and \ref{thm:convergencerates}). Finally, the regret (upper and lower) bounds for the symmetric range are discussed in Section~\ref{sec:symmetric} (Theorems~~\ref{thm:expert-regret-bound-symmetric}, \ref{thm:expert-log-dependency-symmetric}, \ref{thm:bandit-regret-bound-symmetric}, and \ref{thm:bandit-lower-bound-symmetric}).
  

